Rank Diminishing in Deep Neural Networks

The rank of neural networks measures information flowing across layers. It is an instance of a key structural condition that applies across broad domains of machine learning. In particular, the assumption of low-rank feature representations leads to algorithmic developments in many architectures. For neural networks, however, the intrinsic mechanism that yields low-rank structures remains vague and unclear. To fill this gap, we perform a rigorous study on the behavior of network rank, focusing particularly on the notion of rank deficiency. We theoretically establish a universal monotonic decreasing property of network rank from the basic rules of differential and algebraic composition, and uncover rank deficiency of network blocks and deep function coupling. By virtue of our numerical tools, we provide the first empirical analysis of the per-layer behavior of network rank in practical settings, i.e., ResNets, deep MLPs, and Transformers on ImageNet. These empirical results are in direct accord with our theory. Furthermore, we reveal a novel phenomenon of independence deficit caused by the rank deficiency of deep networks, where classification confidence of a given category can be linearly decided by the confidence of a handful of other categories. The theoretical results of this work, together with the empirical findings, may advance understanding of the inherent principles of deep neural networks.

==> sections/7.1.ack.tex <==
\begin{ack}
%
\vspace{5pt}\textbf{Acknowledgements.}
%
\end{ack}

==> sections/8.checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section xx.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerNo{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{Proofs are included in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> sections/theory_old.tex <==
\section{Principle of Rank Deficiency}\label{sec:method}
We consider the general deep neural network, which is a smooth vector value function $\bm{f}:\mathbb{R}^n\rightarrow\mathbb{R}^d$, where $\mathbb{R}^n$ and $\mathbb{R}^d$ are the ambient space of input and output. Deep neural networks are coupling of multiple layers, thus we write $\bm{f}$ as:
\begin{equation}
    \bm{f}=\bm{f}^1\circ\bm{f}^2\circ...\circ\bm{f}^L.
\end{equation}
Previous works about rank deficiency are mostly built upon specification to the form of $\bm{f}_i,i=1,...,L$, like MLP or Attention with skip connections. In pursuing a more general application, here we only assume $\bm{f}_i$ to be \textit{locally Lipschitz}.


The purpose of this paper is then to show that, the rank of networks and feature manifolds, will decrease monotonously as layer gets deeper. Below we will demonstrate it from a theoretical perspective following by a experimental validation. Before we step into the arguments, there are some primary concepts need to provide for the self-containing.


\paragraph{Rank of Function} Rank of a function $\bm{f}$ refers to the rank of its Jacobi matrix $J_{\bm{f}}$, which is defined as 
\begin{equation}
    rank(\bm{f})=rank(J_{\bm{f}})=rank(\left(\frac{\partial\bm{f}_i }{\partial \x_j}(\x)\right)_{n\times d}).
\end{equation}

\paragraph{Intrinsic Dimension of Feature Manifold} By the rank theorem of manifold and the Sard's Theorem, the rank of a function is also the intrinsic dimension of the manifold it induce.
\begin{lemma}[Sard's Theorem \cite{hirsch2012differential}]\label{lemma: Jacobi}
Let $f:\mathbb{R}^n\rightarrow\mathbb{R}^m$ and $f(\mathcal{Z})=\mathcal{X}^{d_f}$ be a manifold embedded in $\mathbb{R}^m$ with $\mathcal{Z}$ an open subset of $\mathbb{R}^n$. Then for almost every point $x\in\mathcal{X}^{d_f}$, the gradient matrix of $f$ has constant rank $rank(J_{z}f)$ at the pre-image of $x$ in $\mathcal{Z}$, and the intrinsic dimension of $\mathcal{X}^{d_f}$ is $d_f=rank(J_zf)$.
\end{lemma}

\paragraph{Numerical Rank} Numerically, estimation of matrix ranks \cite{ubaru2016fast} relies on calculating the number of eigenvectors that larger than some threshold $\epsilon$, which tolerates the significance of noise perturbations to the matrices. Thus we may estimate the rank of a matrix $W$ in $\mathbb{R}^{n\times d}$ as
\begin{equation}
    rank_{\epsilon}(W)=\vert\{i\in\mathbb{N}_+: i\leq min\{n,d\}, \vert\lambda_i\vert\geq\epsilon\}\vert.
\end{equation}


\subsection{First Law of Rank Deficiency}
Our first result gives a universal justification for the rank deficiency in deep networks. It comes from the basic rule of matrix multiplication and chain rule. We first investigate a trivial result of rank in matrix multiplication.
\begin{lemma}
For any two matrices $\bm{A}\in\mathbb{R}^{n\times m}$ and $\bm{B}\in\mathbb{R}^{m\times d}$, the rank of their multiplication is lower than any of them, \ieno, 
\begin{equation}
    rank(AB)\leq \min\{rank(A),rank(B)\}.
\end{equation}
\end{lemma}
To give an intuitive understanding of the possibility of losing rank after matrix multiplication, it is important to know the mechanism behind this Lemma. For a matrix $\bA$, let $Ker(\bA)=\{\bv:\bA\bv=\bm{0}\}$, \ieno, the space orthogonal to the rows of $\bA$, $Im(\bB)=\{\y:\y=\bB\bv\}$, \ieno, space spanned by the columns of $\bB$, then we have
\begin{lemma}
For any matrices $\bA$ and $\bB$, we have
\begin{gather}
    rank(\bA\bB)=rank(\bB)-dim(Ker(\bA)\cap Im(\bB))\\
    =rank(\bA)-dim(Ker(\bA^T)\cap Im(\bB^T)).
\end{gather}
Thus, if and only if $Ker(\bA)\cap Im(\bB)=\emptyset$, we have $rank(\bA\bB)=rank(\bB)$, otherwise we have $rank(\bA\bB)<rank(\bB)$.
\end{lemma}


\begin{theorem}
Let $\f:\mathbb{R}^n\rightarrow\mathbb{R}^d$ be a deep neural network composed of $L$ layers of sub-networks as
\begin{equation}
    \f=\f_1\circ\f_2\circ...\circ\f_L.
\end{equation}
Suppose each sub-network $\f_i,i=1,...,L$ is differentiable, then we have
\begin{equation}
    rank(\f_1)\geq rank(\f_1\circ\f_2) \geq ...\geq rank(\f_1\circ...\circ\f_{L-1})\geq rank(\f),
\end{equation}
where $rank(\f_i)$ is the rank of the Jacobi Matrix of function $\f_i,i=1,...,L.$ By Sard's theorem, rank of function is \textit{a.e.} the dimension of the manifold it induced, we can also have
\begin{equation}
    dim(\mathcal{F}_1)\geq dim(\mathcal{F}_2)\geq...\geq dim(\mathcal{F}_L),
\end{equation}
where $\mathcal{F}_i=\f_1\circ...\circ\f_i(\mathbb{R}^n), i=1,...,L$ is the feature space induced by the composition of the top-$i$ network layers.
\end{theorem}




\subsection{Second Law of Rank Deficiency}
Assuming that elements of $W$ are sampled from some \textit{i.i.d} distributions, the following two well known results give estimations to the probability of $W$ not having full rank.

\begin{theorem}[Marchenko-Pastur distribution\cite{chen2005condition,edelman1988eigenvalues}]
Let the elements of $W$ be sampled \textit{i.i.d} from the Standard Gaussian, and $\lambda_{min}$ be the eigen value of $W$ with the smallest absolute value. The pdf of $\lambda_{min}$ is given by
\begin{equation}
    p_{\lambda_{min}}(x)=\frac{n}{2^{n-1/2}}\frac{\Gamma(n)}{\Gamma(n/2)}x^{-1/2}e^{-xn/2}U(\frac{n-1}{2}, -\frac{1}{2}, \frac{\lambda}{2}).
\end{equation}
When $a>0$ and $b<1$, the Tricomi function, $U(a,b,z)$ is the unique solution to Kummer's equation
\begin{equation}
    z\frac{d^2w}{dz^2}+(b-z)\frac{dw}{dz}-aw=0
\end{equation}
satisfying $U(a,b,0)=\Gamma(1-b)/\Gamma(1+a-b)$ and $U(a,b,\infty)=0$.
\end{theorem}


The equal sign stands when the subsequent network layer drops zero information, \textit{i.e.}, the layer Jacobi matrix has full rank. This however, may hardly be always true in a deep neural network as the following theorem.
\begin{theorem}[Marchenko-Pastur distribution\cite{chen2005condition,edelman1988eigenvalues}]
Let the elements of $W\in\mathbb{R}^{n\times d}$ be sampled \textit{i.i.d} from the Standard Gaussian, and $\rho(W)=\inf_{x} \frac{\Vert Wx\Vert_2}{\Vert x\Vert_2}$, \textit{i.e.} the eigenvalue with the smallest absolute value. Then there exists a positive constant $C$ that depends on $n,d,\epsilon$, such that
\begin{equation}
    p(rank(W)<min\{n,d\})=p(\rho(W)<\epsilon)>C>0.
\end{equation}
\end{theorem}

\subsection{Third Law of Rank Deficiency}


Bengio \textit{et. al.} discuss the gradient explosion issue of Recurrent Neural Network (RNN) in the classical work \cite{bengio1994learning,pascanu2013difficulty}. Following their settings, consider a RNN $\bm{R}(\x)=\bm{c}\circ\bm{r}\circ\bm{r}...\bm{r}(\x)=\bm{c}(\bm{r}^L(\x))$, which is composed of $L$ recurrent layer $\bm{c}$ to get the 
feature representation of data $\x$, and a dense layer $\bm{c}$ to output the confidence score for sample $\x$. Let $\sigma_1,\sigma_2,...,\sigma_n$ be the eigenvalues of the layer Jacobi $\bJ_{\bm{r}}$ sorted by their magnitudes, $\bm{q}_1,...,\bm{q}_n$ be the corresponding normalized eigenvectors. They then show that \cite{pascanu2013difficulty} the differential of representation
\begin{equation}\label{eq:gradient explosion}
     \dx\bm{r}^L(\x)=\bJ_{\bm{r}^L}(\x-\x_0)^T\dx\x=(\bJ_{\bm{r}})^L(\x-\x_0)^T\dx\x=\alpha_1\sigma_1^L\bm{q}_1 \dl{\dx\x}+\sigma_1^L\sum_{i=2}^n\alpha_i(\frac{\sigma_i}{\sigma_1})^L\bm{q}_i\dx\x,
\end{equation}
where $\alpha_i=\langle\dx\x,\bm{q}_i\rangle,i=1,...,n$. Thus when the depth of network $L\rightarrow\infty$, we have $(\frac{\sigma_i}{\sigma_1})^L\rightarrow0$ and $\dx\bm{r}^L(\x)\approx\alpha_1\sigma_1^L\bm{q}_1\dx\x$. If $\vert\sigma_1\vert>1$, the differential explodes exponentially; if $\vert\sigma_1\vert<1$, it vanishes exponentially. Various tools like ResNet, Skip Connections, Relu, \etcno., are then invented to address this issue. However, the rank diminishing issue behind this gradient issue is neglected long in the community. \cref{eq:gradient explosion} also implies monotonously decreasing of the numerical rank of the network Jacobi, and when layer depth $L>\log n\epsilon / \log\frac{\sigma_2}{\sigma_1}$, $\rank_{\epsilon}(\bJ_{\bm{r}^L})=1$ \dl{connection with~\cite{Dong@rankCollapse2021}} , thus the feature representation $\bm{r}^l(\x)$ degenerates to a $1$ dimensional space. 

To see the damage this degeneration can cause, consider the classification task in ImageNet, where $\bm{R}=(\bm{R}_1,...,\bm{R}_{1000})^T$ is a 1,000 dimensional vector with each dimension indicates the classification probability to a ImageNet category. Then we have 
\begin{equation}
\begin{aligned}
        \bm{R}_i(\x)-\bm{R}_i(\x_0)\approx \dx\bm{R}_i =\frac{\dx\bm{c}_i}{\dx\bm{r}^L}\dx\bm{r}^L=(\nabla_{\bm{r}^L}\bm{c}_i)^T(\alpha_1\sigma_1^L\bm{q}_1+\sigma_1^L\sum_{i=2}^n\alpha_i(\frac{\sigma_i}{\sigma_1})^L\bm{q}_i)\dx\x\\
        \approx\alpha_1\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_i,\bm{q}_1\rangle=(\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_i,\bm{q}_1\rangle)\bm{q}_1^T\x,i=1,...,n.
\end{aligned}
\end{equation}
Note that $(\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_i,\bm{q}_1\rangle)$ and $\bm{R}_i(\x_0)$ are locally data independent constants, thus the classification probability of any two independent categories $i,j$ of any point $\x$ nearby $\x_0$ are actually decided by each other
\begin{equation}
    % \bm{R}_i(\x)=\frac{\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_i,\bm{q}_1\rangle}{\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_j,\bm{q}_1\rangle}\bm{R}_j(\x)
    \bm{R}_i(\x)=\xi\bm{R}_j(\x)+\gamma,
\end{equation}
with $\xi=\frac{\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_i,\bm{q}_1\rangle}{\sigma_1^L\langle\nabla_{\bm{r}^L}\bm{c}_j,\bm{q}_1\rangle}$ and $\gamma=\bm{R}_i(\x_0)-\xi\bm{R}_j(\x_0)$. Thus for any image of ImageNet, its possibilities of being ostrich, turtle, dogs, cats, birds, \etcno., will be all decided by its possibility of being tank, which is obviously absurd.

